Scalable Multi-Domain Adaptation of Language Models using Modular Experts

Domain-specific adaptation is critical to maximizing the performance of pre-trained language models (PLMs) on one or multiple targeted tasks, especially under resource-constrained use cases, such as edge devices. However, existing methods often struggle to balance domain-specific performance, retention of general knowledge, and efficiency for training and inference. To address these challenges, we propose Modular Domain Experts (MoDE). MoDE is a mixture-of-experts architecture that augments a general PLMs with modular, domain-specialized experts. These experts are trained independently and composed together via a lightweight training process. In contrast to standard low-rank adaptation methods, each MoDE expert consists of several transformer layers which scale better with more training examples and larger parameter counts. Our evaluation demonstrates that MoDE achieves comparable target performances to full parameter fine-tuning while achieving 1.65% better retention performance. Moreover, MoDE's architecture enables flexible sharding configurations and improves training speeds by up to 38% over state-of-the-art distributed training configurations.

==> Makefile <==
LATEX := pdflatex

all: paper.pdf

BIB := $(shell find . -name '*.bib')
FIGS := $(shell find figures/ -name '*.pdf')
TIKZ := $(shell find figures/ -name '*.tikz')
TEX := $(shell find . -name '*.tex')
EXTS = *.aux *.backup *.blg *.log *.out *.lof *.loa *.lot *.toc *.bak \
       *.texshop *.dvi *.fdb_latexmk *.fls *.ent *.run.xml *.run.xml

paper.pdf: ${TEX}  ${TIKZ} ${BIB} ${FIGS}
	latexmk -pdf -bibtex paper.tex

clean:
	latexmk -C
	rm -f paper.pdf
	rm -f ${EXTS}



==> related-work.tex <==
\section{Related Work}
\label{s:related-work}

\textbf{Mixture-of-Experts (MoE)}: Models employing the mixture-of-experts architecture, explored in~\cite{shazeer2017outrageously,zadouri2023pushing, du2022glam, lepikhin2020gshard,
zhou2022mixtureofexperts}, demonstrate superior scaling properties. For any given input, only a subset of experts is activated, leading to improved computational efficiency while maintaining or improving model performance. LoRAMoE~\cite{dou2023loramoe} innovates on the MoE concept by focusing on maintaining up-to-date knowledge within the language model's framework.
Although being extremely efficient in training, MoE does not address
serving efficiency as discussed in Section~\ref{subsec:coarse_routing}.

\textbf{Parameter-Efficient Transfer Learning}: Traditionally, full fine-tuning is critical for adapting pretrained language models. Due to the immense size of LLMs, parameters-efficient fine-tuning have become prevalent~\cite{hu2021lora,liu2022fewshot,li2021prefixtuning}. Techniques like conditional adapters~\cite{lei2023conditional}, AdaMix~\cite{wang2022adamix}, and
MixPHM~\cite{jiang2023mixphm} specialize parts of a pre-trained LLM's
parameters to learn new tasks or adjust to different domains,  This
strategy dramatically reduces the model size as compared to full
fine-tuning. These methods aim to inject domain knowledge or adapt the LLM
without modifying the large body of its original parameters.

\textbf{Low-Rank Adaptation (LoRA)}: LoRA~\cite{hu2021lora} and QLoRA~\cite{dettmers2023qlora} offers a
promising approach to enhancing LLM performance by introducing trainable
rank-decomposition matrices into the model architecture. Unlike traditional
adapters, which can incur significant latency during inference, LoRA
maintains model efficiency while achieving comparable or even superior
results. However, LoRA has limited expressiveness, limiting its
effectiveness on complex tasks~\cite{anyscale-finetuning-lora}.


